Deep OCT Angiography Image Generation for Motion Artifact Suppression

Eye movements, blinking and other motion during the acquisition of optical coherence tomography (OCT) can lead to artifacts, when processed to OCT angiography (OCTA) images. Affected scans emerge as high intensity (white) or missing (black) regions, resulting in lost information. The aim of this research is to fill these gaps using a deep generative model for OCT to OCTA image translation relying on a single intact OCT scan. Therefore, a U-Net is trained to extract the angiographic information from OCT patches. At inference, a detection algorithm finds outlier OCTA scans based on their surroundings, which are then replaced by the trained network. We show that generative models can augment the missing scans. The augmented volumes could then be used for 3-D segmentation or increase the diagnostic value.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% Horsch 041224
%
% - übernommen von Lehmann
% - angepasst für Proceedings BVM2003, Erlangen, Jan 2003
%	- Pseudo-Definitionen für tocgenerate (Generierung Inhaltsverz.)
%   \pagecount (Dez 2004)
%

\catcode`@=11

\def\makeauthor{\if@filesw \newwrite\@aindexfile
  \immediate\openout\@aindexfile=\jobname_authors.pix
  \def\addauthor{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wraindex}\typeout
  {Writing index file \jobname_authors.pix }\fi}

\def\@wraindex#1{
   \edef\@tempa{\write\@aindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addauthor{\@bsphack\begingroup \@sanitize\@addauthor}

\def\makepreindex{\if@filesw \newwrite\@pindexfile
  \immediate\openout\@pindexfile=\jobname_index.pix
  \def\addpreindex{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wrpindex}\typeout
  {Writing index file \jobname_authors.pix }\fi}

\def\@wrpindex#1{
   \edef\@tempa{\write\@pindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addpreindex{\@bsphack\begingroup \@sanitize\@addpreindex}

\def\makecategory{\if@filesw \newwrite\@bindexfile
  \immediate\openout\@bindexfile=\jobname_category.pix
  \def\addcategory{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wrbindex}\typeout
  {Writing index file \jobname_category.pix }\fi}

\def\@wrbindex#1{
   \edef\@tempa{\write\@bindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addcategory{\@bsphack\begingroup \@sanitize\@addcategory}

\catcode`@=12




% \newcommand{\tocentry}[7]
\newcommand{\tocentry}[5]
% #1 = articletype + counter
% #2 = title
% #3 = Autoren
% #4 = Autoren, erster fett
% #5 = Seitenzahl
           {
            %\vspace{3mm}
            \noindent
%ho            \begin{minipage}[b]{115.5mm}
            \begin{minipage}[b]{114.5mm}
            \raggedright
            \begin{list}{}{\labelwidth9mm
                           \leftmargin9mm
                           \labelsep0mm}
%ho            \item[#1 \hfill] #3 \newline
%ho                        {\em #4}\dotfill
%             \item[#1 \hfill] {\em #2:} #4 #3 \dotfill
            \item[#1 \hfill] #3: #2 \dotfill  % #1 = Buchstabe und lfd. Nr.; #2 = Autoren; #3 = Autoren ;#4 = Titel
            \end{list}
            \end{minipage}
%ho            \begin{minipage}{5.5mm}
            \begin{minipage}{6.5mm}
%             \hfill\raisebox{1.5pt}{\the\tocpos} % Seitennummer
%             \hfill\raisebox{1.5pt} 
	      \hfill \raisebox{1.5pt}{#5}
            \end{minipage}
%             \addauthor{#5}
%             \addpreindex{#7}
%             \addcategory{#6}
%             \advance \tocpos #2\relax % advance erhöht/vermindert die Variable tocpos; relax macht nichts (no-op) = Abbruch ohne Fehlermeldung
%             \advance \tocpos \relax % advance erhöht/vermindert die Variable tocpos; relax macht nichts (no-op) = Abbruch ohne Fehlermeldung
        }


\newcommand{\firma}[1]
           {\begin{minipage}[t]{58mm}
             #1
            \end{minipage}}

\newcommand{\siehe}[2]{#2, {\it siehe} #1}

\newcommand{\nachsatz}[2]{#1, #2}

\newcommand{\nachsatzfett}[2]{#1, {\bf #2}}

\newcommand{\fett}[1]{{\bf #1}}

\newcommand{\fettumbruch}[1]{{\bf #1} \newpage}

\newcommand{\umbruch}[1]{#1 \newpage}

\newcommand{\zwischen}[1]
           {\newpage
            \rule{0mm}{0mm}

            \vspace{5cm}
            \begin{center}
            \baselineskip35pt
            {\huge \bf #1} 
            \end{center}}

%	Pseudo-Definition für tocgenerate
\newcommand{\pagecount}[1]{}


\newcommand{\elqq}{``}%
\newcommand{\erqq}{''}%
